TransResU-Net: Transformer based ResU-Net for Real-Time Colonoscopy Polyp Segmentation

Colorectal cancer (CRC) is one of the most common causes of cancer and cancer-related mortality worldwide. Performing colon cancer screening in a timely fashion is the key to early detection. Colonoscopy is the primary modality used to diagnose colon cancer. However, the miss rate of polyps, adenomas and advanced adenomas remains significantly high. Early detection of polyps at the precancerous stage can help reduce the mortality rate and the economic burden associated with colorectal cancer. Deep learning-based computer-aided diagnosis (CADx) system may help gastroenterologists to identify polyps that may otherwise be missed, thereby improving the polyp detection rate. Additionally, CADx system could prove to be a cost-effective system that improves long-term colorectal cancer prevention. In this study, we proposed a deep learning-based architecture for automatic polyp segmentation, called Transformer ResU-Net (TransResU-Net). Our proposed architecture is built upon residual blocks with ResNet-50 as the backbone and takes the advantage of transformer self-attention mechanism as well as dilated convolution(s). Our experimental results on two publicly available polyp segmentation benchmark datasets showed that TransResU-Net obtained a highly promising dice score and a real-time speed. With high efficacy in our performance metrics, we concluded that TransResU-Net could be a strong benchmark for building a real-time polyp detection system for the early diagnosis, treatment, and prevention of colorectal cancer. The source code of the proposed TransResU-Net is publicly available at https://github.com/nikhilroxtomar/TransResUNet.

==> out.tex <==

% \section*{Acknowledgement}
% D. Jha is funded by  Research Council of Norway project number 263248 (Privaton). The computations in this paper were performed on equipment provided by the Experimental Infrastructure for Exploration of Exascale Computing (eX3), which is financially supported by the Research Council of Norway under contract 270053.

Figure~\ref{fig:proposed-architecture} show the block diagram of our proposed TResU-Net. The proposed architecture follows an encoder-decoder scheme, where we have four encoder blocks and four decoder blocks. The input image is fed to the first encoder block, which begins with a residual block~\cite{he2016deep} and a $2\times2$ max-pooling layer, where the spatial dimensions of the feature maps are reduced to half. Subsequently, the output from the first encoder block is passed to the next encoder blocks and finally, the output of the last encoder block is passed through a transformer encoder block and a dilated convolution block. The transformer encoder block~\cite{vaswani2017attention} consists of a self-attention network which is followed by a feed-forward network. While the dilated convolution block consists of four parallel $3\times3$ convolution layers, where each layer has a dilation rate of $1$, $3$, $6$ and $9$ respectively. These layers are then followed by batch normalization and a ReLU activation function. Next, we concatenate the features from all the four layers and pass them through a $1\times1$ convolution layer. The output from both the transformer encoder block and the dilated convolution block is concatenated and passed to the first decoder block. The decoder block begins with a bilinear upsampling, which is followed by the concatenation with the skip connection from the encoder block. The concatenated feature maps are then passed through two residual blocks, which act as the output of the decoder block. The output from the last decoder block is passed through a $1\times1$ convolution layer followed by a sigmoid activation function which generates a binary segmentation mask.


% \begin{table*}[t!]
% \centering
% \caption{Quantitative results of TresResU-Neton Kvasir-SEG~\cite{jha2020kvasir}}
%  \begin{tabular} {@{}l|c|c|c|c|c|c|c@{}}
% \toprule
% \textbf{Method} &\textbf{Image size} & \textbf{F1} & \textbf{mIoU} &\textbf{Recall}  &\textbf{Precision}& \textbf{Accuracy}  &\textbf{FPS}\\ 
% \hline
% RUPNet	&$512\times 512$	&0.7673 &0.6822	&0.7784 &0.8595 &0.9434 & 85.35\\
% \bottomrule
% \end{tabular}
% \label{tab:results}
% \end{table*}

% The input image is fed to the first encoder block, which begins with a residual block consisting of two $3\times3$ convolution layers, each followed by batch normalization and a ReLU activation function. After that, it is followed by an identity mapping (residual connection) connecting the input and output of the convolutional layers. The output from the residual block is then passed through a $2\times2$ max-pooling layer, where the spatial dimensions (height and width) of the feature maps are reduced to half. 

% The transformer encoder block consists of a self-attention which is followed by a feed-forward network which helps the network to extract more useful features and produce a robust feature representation. 

% These skip connections help in the flow of information from the encoder to the decoder block, which helps in generating better semantic features.


%Deep learning based algorithm showed promising results than traditional machine learning based algorithm because of their capability to extract features from input images. Deep learning based algorithm also reduce the diagnosis time and computational resource which is associated to patient safety. 
